Masked Imitation Learning: Discovering Environment-Invariant Modalities in Multimodal Demonstrations

Multimodal demonstrations provide robots with an abundance of information to make sense of the world. However, such abundance may not always lead to good performance when it comes to learning sensorimotor control policies from human demonstrations. Extraneous data modalities can lead to state over-specification, where the state contains modalities that are not only useless for decision-making but also can change data distribution across environments. State over-specification leads to issues such as the learned policy not generalizing outside of the training data distribution. In this work, we propose Masked Imitation Learning (MIL) to address state over-specification by selectively using informative modalities. Specifically, we design a masked policy network with a binary mask to block certain modalities. We develop a bi-level optimization algorithm that learns this mask to accurately filter over-specified modalities. We demonstrate empirically that MIL outperforms baseline algorithms in simulated domains including MuJoCo and a robot arm environment using the Robomimic dataset, and effectively recovers the environment-invariant modalities on a multimodal dataset collected on a real robot. Our project website presents supplemental details and videos of our results at: https://tinyurl.com/masked-il

==> sections/01.short_intro.tex <==


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/teaser.pdf}
   % \includesvg[width=1.25\textwidth]{figures/overview.svg}
    \vspace{-0.5cm}
    \caption{\small{An illustrative overview of masked imitation learning from multimodal data: we want to learn modality masks for selecting the input modalities that are invariant across different environments. In this example of transferring policies from sim to real, RGB modality has a larger domain gap than depth and proprioception. Masked imitation learning (MIL) would would learn to mask out the RGB modality because it induces lower loss on the real-world data using policies trained on sim data. }}
    \label{fig:overview}
    \vspace{-0.5cm}
\end{figure*}


%===============================================================================

\section{Introduction}
\label{sec:introduction}
% More modalities, more capable robots
Humans are born with the ability to perceive and integrate multiple sources of sensory information, including vision, touch, sound, and proprioception. 
Cognitive science research has demonstrated that humans form a coherent and robust perception of the world by efficiently integrating multiple sensory information~\cite{ernst2004merging,stein1993merging}. 
A robust perception is the foundation for sensorimotor control.
To mimic human sensing, modern robotic systems are often equipped with multitudes of sensors.  
Such \textit{multimodal} sensory information is important for solving robotics tasks~\cite{calandra2018more,zhang2019leveraging,mu2021maniskill}. 


Multimodal sensory data provides abundant information for decision making and much research effort has been dedicated to developing better robot sensing capabilities~\cite{liu2019flexible,abad2020visuotactile,dai2022design}. 
\textbf{However, somewhat unintuitively, more data modalities do not necessarily promise higher performance for sensorimotor policies learned from such data.}
Multiple prior works have observed that when learning from multimodal sensory data, using a subset of input modalities can lead to better task performance than using all modalities~\citep{janner2019trust,xiao2020multimodal,mandlekar2021matters,tomar2021model}.
This phenomenon is caused by \textit{state over-specification}---the state contains extraneous data modalities that do not provide useful information for solving the task but can introduce a different data distribution across environments.
Consider the example in Fig.~\ref{fig:overview}, a robot is trained to perform a pick-and-place task in simulation from three different modalities (RGB image, depth image, and proprioception). To locate and pick up the object, depth and proprioception information are sufficient. The remaining modality of RGB image that changes from simulation to the real setting over-specifies the state for this particular task.
When such extraneous information is used by learned policies to predict action, they are less likely to generalize at test time, especially when the testing environment changes, e.g., when training in simulation and testing the policy on the real robot (see Fig.~\ref{fig:overview}). 
Prior work in learning from multimodal data only focuses on fusing various sensory modalities~\cite{akinola2020learning,liu2017learning,mu2021maniskill,lee2020making,lee2021detect,xiao2020multimodal}, but do not explicitly address the potential state over-specification problem.
In this paper, we focus on addressing this problem to avoid overfitting to training data when learning from multimodal data.
Going back to the example in Fig.~\ref{fig:overview}, 
if we remove the RGB modality, the robot still has sufficient information for performing the task and now the testing input looks more aligned with training data such that policy trained in simulation may generalize to the real environment.
Our key insight is that, for a particular task, we need to be \textit{selective} about what modalities the policy relies on for decision-making to avoid state over-specification.

We propose Masked Imitation Learning~(\textbf{MIL}), which learns a binary mask for each modality to decide whether the modality should be used for action prediction. 
MIL is a bi-level optimization algorithm: in the inner-level, MIL learns a policy embedded with a fixed mask on the training datasets using the training loss; in the outer-level, MIL updates the mask according to the validation loss evaluated on the validation dataset for the policy learned for each mask in the inner loop. The validation loss selects a policy that generalizes well to the validation dataset, which is more likely to be learned with no over-specified modalities, i.e. the corresponding mask removes over-specified modalities. We demonstrate the effectiveness of MIL empirically on several robotic tasks both in simulation including existing robotics datasets such as Robomimic~\cite{mandlekar2021matters} and on multimodal data collected for a real robot manipulation task.
We show learning from a selected set of modalities can improve the performance by 5.6$\times$ than learning from all modalities in certain domain.
%Specifically, our contributions are:
%\begin{itemize}[leftmargin=*]
%\vspace{-0.25cm}
%    \setlength\itemsep{-0.25em}
%    \item identifying and formalizing the state over-specification problem in learning from multimodal data;
%    \item developing a bi-level optimization algorithm, masked imitation learning (MIL), which learns a policy for each mask in the inner loop and selects a binary modality mask using the coordinate descent algorithm according to the validation loss of the inner loop policy for the outer loop;
%    \item demonstrating the effectiveness of
%MIL empirically on several robotic tasks both in simulation including when using existing robotics datasets such as Robomimic and on multimodal data collected for a real robot manipulation task.
%\end{itemize}




==> sections/02.short_related_work.tex <==

%===============================================================================

\section{Related Work}

Our work addresses the state over-specification problem experienced by imitation learning from multimodal sensory data and therefore 
is closely related to prior work in \textit{learning from multimodal sensory data}, \textit{imitation learning}, and the broad area of \textit{invariant representation learning}. 
%In additiona, state over-specification leads to overfitting, which has been extensively studied under the idea of \textit{invariant representation learning}.

\medskip

\noindent \textbf{Learning from Multimodal Sensory Data.} 
Motivated by the potential of leveraging information from multiple sensory modalities, prior works have explored using multimodal data for robot learning.
These works mainly focus on what data modalities should be included for robot learning, where single-view images~\cite{lee2020making,calandra2018more,gao2016deep}, multi-view images~\cite{akinola2020learning}, haptic data~\cite{bekiroglu2011learning,calandra2018more,gao2016deep,sinapov2014learning}, range sensing~\cite{liu2017learning,sung2017learning}, audio~\cite{du2022play,zhang2019leveraging,dean2020see}, depth images~\cite{lee2020making} and 3D point clouds~\cite{mu2021maniskill} are adopted to learn different manipulation and navigation tasks. 
These works demonstrate that, for a given task, one can leverage a comprehensive set of modalities to provide the necessary information for decision-making.
Prior works have also investigated how to learn a robust state representation from multimodal sensory data using auxiliary objectives for better test-time generalization~\cite{yang2017deep,chen2021multi,lee2020making,lee2021detect}. 
Finally, a growing body of work also focuses on using multimodal data to learn end-to-end sensorimotor policies~\cite{ernst2004merging,liu2017learning,lee2020making,xiao2020multimodal,akinola2020learning,mu2021maniskill,du2022play}.
However, all these works utilize all the available modalities and do not consider the state over-specification problem that can occur due to extraneous modalities. 
We show that overfitting --- while being overlooked by most prior works --- is a common problem when learning from multimodal data, and we address it by our masked imitation learning approach. 

\medskip

\noindent \textbf{Imitation Learning.} 
Imitation learning aims to learn a policy from demonstrations~\cite{argall2009survey,osa2018algorithmic}. Behavioral cloning~\cite{bain1995framework} is the simplest form of imitation learning that treats the problem as supervised learning but often suffers from compounding errors at test time since the test data is not independent and identically distributed (i.i.d.).
More advanced imitation learning techniques such as generative adversarial imitation learning simultaneously learn a discriminator and the policy, addressing overfitting by rolling out the learned policies and applying a discriminative loss on agent trajectories that are far from those in demonstrations~\cite{schroecker2017state,torabi2018generative,sun2019provably,fu2017learning}. 
Further, several recent methods explicitly address the distribution shift between the demonstrations and the imitation agent's policy rollouts~\cite{liu2019state,cao2021corl}.
However, rolling out agent policies is not only expensive but also often unsafe for real-world robotics applications. 
In contrast, our algorithm learns from offline data and does not need to iteratively interact with the environment, and at the same time can be easily adapted to learn the environment-invariant modality mask in an online manner.


%\textbf{Invariant Risk Minimization.} 
\noindent \textbf{Invariant Representation Learning.} 
Deep neural networks are known to have the capacity to memorize noise or pick up spurious correlations~\cite{zhang2021understanding,arpit2017closer}.
To reduce environment-specific overfitting, techniques including invariant risk minimization~\cite{arjovsky2019invariant,mahajan2021domain}, self-training~\cite{chen2020self,xie2020self}, dropout~\cite{srivastava2014dropout} and feature selection~\cite{yang1997comparative,bach2008bolasso,urbanowicz2018relief} are proposed to focus more on features with causal relationships to the outcome. However, all of these methods are only verified for non-robotics tasks.
%However, for imitation learning, we need to focus on reducing the spurious features in the states that are correlated with the action outcome. 
For robotics tasks, several works propose information bottleneck to learn the task-relevant representation, which is invariant across domains~\cite{pacelli2020learning,lu2020dynamics}, but these approaches require a well-defined reward and interactions with the environment. Invariant risk minimization games is a theoretical framework to learn an invariant policy in many different environments to reduce the effect of spurious features~\cite{ahuja2020invariant}.
However, creating the set of environments that capture all the variations of spurious features is quite challenging especially in robotics domains. To address this, domain randomization approaches~\cite{tobin2017domain,peng2018sim,bousmalis2018using} try creating diverse environments by randomizing factors such as texture, lighting, etc., but a large number of variations of these factors, which often need to be done in simulation, might still not be able to capture all the spurious features. 
%Inspired by the ideas in invariant risk minimization, we take advantage of the problem structure of learning from multimodal data and the explicit notion of different training and validation environments. 
Inspired by the idea of invariant risk minimization that explicitly leverages the notion of \textit{environments}, our proposed method learns to mask out extraneous modalities that lead to poor generalization error in the validation environment so that our learned policies do not suffer from overfitting. 




% The idea of Invariant policy optimization generalizes the ideas in IRM to model-based reinforcement learning setting.

%Our goal is similar to that of IRM but we exploit the structure of multimodal imitation learning to address the overfitting problem.


%\textbf{Guided feature learning} In classical machine learning, a domain expert would engineer the features for an algorithm so that it leverages all the necessary and sufficient information.
%Recent work in robot learning from humans has looked at human-guided feature learning.

%In our problem setting, we assume no access to the human expert during learning and limited access to the task environment. 


==> sections/03.short_method.tex <==

\section{Problem Setting}
\label{sec:problem}

We consider sequential decision-making problems modeled as Markov Decision Processes (MDPs). 
An MDP is defined by the tuple  $\langle \mathcal{S,A,T,R} \rangle$, where:
    $\mathcal{S}$ and $\mathcal{A}$ are the state space and action space; 
    $\mathcal{T}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S} $ is a transition probability function; and
     $\mathcal{R}$ is a reward function. 
Here, we focus on deterministic MDPs but as we discuss in the Appendix, our method can be easily extended to the stochastic case.
In this paper, we focus on the setting where the state space $\mathcal{S}$ consists of $M$ modalities: $\mathcal{S}=\bigtimes_{i=1}^{M}\mathcal{S}^i$, where each $\mathcal{S}^i$ indicates the state space of a modality.
A trajectory %$\tau = \{(s^i_0|_{i=1}^{M},a_0),(s^i_1|_{i=1}^{M},a_1),...,(s^i_n|_{i=1}^{M},a_n)\}$ is a sequence of state-action pairs, where $s^i_t$ indicates the state of modality $i$ at time step $t$. 
$\tau = \{(s_0,a_0),(s_1,a_1),...,(s_n,a_n)\}$ is a sequence of state-action pairs, where every state at time $t$ has $M$ modalities $s_t = [s^0_t,...,s^M_t]$.
The return of a trajectory is the sum of rewards $\sum_{t=0}^n[\mathcal{R}(s^i_t|_{i=1}^{M},a_t)]$.
% A policy $\pi$ maps from states to actions. Solving an MDP involves finding a policy that achieves maximum return. 
Let $e \in \mathcal{E}$ denote an environment, which we define as a subspace of states $\mathcal{S}_e \subset \mathcal{S}$ that are reachable by the transition function $\mathcal{T}$ when initialized at $s_0 \in \mathcal{S}_e$.
% , starting from an initial state $s_0 \in \mathcal{S}_e$.
A policy is a mapping from states to actions, $\pi: \mathcal{S} \rightarrow \mathcal{A}$. Similarly, an expert policy in an environment $e$ is $\pi^E: \mathcal{S}_e \rightarrow \mathcal{A}$ that maximizes the expected return. Expert demonstrations can be sampled from this policy to create a dataset: $\mathcal{D}_e =\{\tau_0,\tau_1,...,\tau_k\}$ of size $|\mathcal{D}_e|$.
% Expert demonstration trajectories $\mathcal{D}_e =\{\tau_0,\tau_1,...,\tau_k\}$ of size $|\mathcal{D}_e|$ are assumed to be collected by an expert with policy $\pi^E$ in the environment $e$. 

The goal of \textbf{imitation learning} is to learn a policy generalizable across environments from multimodal demonstrations. 
Specifically, we have a training environment $e_{\text{train}}$, a validation environment $e_{\text{val}}$, and a testing environment $e_{\text{test}}$. 
Given a training dataset $\mathcal{D}_{\text{train}}$ with $|\mathcal{D}_{\text{train}}|$ demonstrations collected from $e_{\text{train}}$ and a validation dataset $\mathcal{D}_{\text{val}}$ with $|\mathcal{D}_{\text{val}}|$ demonstrations collected from $e_{\text{val}}$, our goal is to learn a policy that achieves high performance in $e_{\text{test}}$ using the data in $\mathcal{D}_{\text{train}}$ and $\mathcal{D}_{\text{val}}$ ($|\mathcal{D}_{\text{train}}|\gg |\mathcal{D}_{\text{val}}|$). %, which means that the validation data is not sufficient for training a well-performing policy. 
We assume that, when providing demonstrations, the expert has access to the same raw state, hence the same data modalities, as the learning agent does.
%The policy $\pi_\theta$'s model capacity is measured by the number of parameters $|\theta|$.

%An agent needs to learn an imitating policy $\pi$ from the demonstrations in training and validation environments $\mathcal{D}_{\text{train}}$, $\mathcal{D}_{\text{val}}$, and achieve performance (return) similar to $\pi^E$ in test environment $e_{\text{test}}$. The policy $\pi$'s model capacity $M$ is measured by the number of parameters.
%\footnote{In practice, the reward function $\mathcal{R}$ for a demonstrated task is often not observed and hence the evaluation of the policy is subjective to the human user/expert's judgement.}

Imitation learning algorithms often learn a policy that minimizes the training loss $\mathcal{L}$ on the training dataset %$\mathcal{D}_{\text{train}}$\footnote{
In practice, this loss function $\mathcal{L}$ is usually the maximum likelihood loss or L2 distance for continuous action spaces or a cross-entropy loss for discrete action spaces.
%}.
% on the training dataset $\mathcal{D}_{\text{train}}$. 
 During training, the best model is selected by validation loss, which is of the same form as the training loss but is evaluated on the validation dataset $\mathcal{D}_{\text{val}}$. \textbf{Overfitting} is a phenomenon that the model learned by the training loss on $\mathcal{D}_{\text{train}}$ and selected by the validation loss on $\mathcal{D}_{\text{val}}$ performs poorly on the test environment $e_{\text{test}}$. 

% \textbf{Overfitting} in imitation learning is the phenomenon that the learned policy achieves low predictive loss $\mathcal{L}_{val}$ on validation data $\mathcal{D}_{val}$ but performs poorly on test environment $\mathcal{E}_{test}$.
%Overfitting can have many different reasons, including the fact that the sequence data in imitation learning is often not independent and identically distributed (i.i.d.) while the algorithms regularly assume access to i.i.d. data.
% nature of imitation learning. 
In this work, we focus on addressing overfitting caused by \textbf{state over-specification}, which happens when the state observed by the imitating agent contains more modalities than what was used by the demonstrator to perform the task, and such modalities change the data distribution across environments. For example, to perform the task of \textit{cutting an apple into slices}, a human demonstrator only needs the location, shape, and size of the apple while the texture of the cutting board or the color of the knife handle is useless and may change in different kitchens. Though both observing the full state information, a human demonstrator selects the useful and generalizable modalities in the state to make decisions, enabling humans to perform the task across environments, but an imitating agent may \textit{overfit} to the over-specified modalities, e.g., if we have only observed knives with green handles in training, the agent at test time can only cut the apple when the knife's handle is green.

%\textbf{Assumptions.} We assume that, when providing demonstrations, 1) the expert has access to the same raw state, hence the same data modalities, as the learning agent does; and 2) the expert makes use of all or a subset of these modalities to decide how to act.

% or when the cutting board looks exactly the same as in training. 

\noindent \textbf{Problem Statement.}  Let $s^i|_{i=0}^M\in \mathcal{S}$ denote the full state with $M$ modalities and $s^i_*|_{i=0}^N\in \mathcal{S^*}$ denote the modalities of size $N$ ($N$$\leq$$M$), which the expert uses to make decisions ($\mathcal{S}^*$ is the environment-invariant modalities for the demonstrated task). 
We let $\bar{s}|_{i=0}^{M-N} \in \bar{\mathcal{S}}$ of size $M-N$ denote the extraneous modalities that are not used by the expert to act.
Our goal is to find a policy $\pi_\theta: \mathcal{S} \rightarrow \mathcal{A}$ trained and validated on $\mathcal{D}_\text{train}$ and $\mathcal{D}_\text{val}$ respectively, which matches the performance of an expert demonstrator $\pi^E: \mathcal{S^*} \rightarrow \mathcal{A}$ in test environment $e_\text{test}$, while the agent observes the full state including the extraneous modalities $\bar{s} \in \bar{\mathcal{S}}$. We define this problem as the state over-specification problem for imitation learning from multimodal data.
% In this work, we address the state-overspecification problem for imitaiton learning from multimodal data, in which the learned $\pi_\theta$ relies on the extraneous modalities $\bar{s}$, beyond what the expert demonstrator has used, to make its prediction and thus leads to poor performance at test time.


%To approach this problem, we first make a few observations about how properties of $\bar{s}$ influences learning.

%\textbf{Remark 0.} Redundant information does not influence learning.


%\textbf{Remark 1.} If modalities in $\bar{S}$ are constants per environment (such as background, lighting, etc.) or only spurious in certain environments, they act as a context for policy learning and overfitting to such states can be reduced by increasing the amount of expert data from different environments.

%\textbf{Remark 2.} If modalities in $\bar{S}$ are spurious in all environments (such as brake indicator, end-effector speed, etc.), observing more expert data will not alleviate overfitting to such states and data from the learned policy is needed to reduce such overfitting.



%Now we first define the correlations under the background of multimodal data and then explain the reason for overfitting.

%\textbf{Correlation.} For an environment $e$, let $S$ is a random variable representing the full state, which takes values from $\mathcal{S}_e$ and $S^i$ is a random variable representing the state of $i$-th modality for $S$, which takes values from $\mathcal{S}^i_e$, then a correlation exists between the $i$-th modality and the expert action if and only if $I(S^i;\pi^E(S))>0$, where $I(\cdot;\cdot)$ is the mutual information between two variables and $\pi^E$ is the expert policy for the environment $e$. Similarly, for a dataset $D$, let $S^i$ is a variable representing the state of the $i$-th modality existing in the dataset, and $A$ as the action binding to $S^i$ in the dataset, then a correlation exists between the $i$-th modality and the action in the dataset if and only if $I(S^i;A)>0$. If a correlation only exists in the training dataset $\mathcal{D}_{\text{train}}$ or $\mathcal{D}_{\text{val}}$ but violates in the test environment $e_\text{test}$, this correlation is a spurious correlation. If a policy relies on the spurious correlations to predict the action, it will overfit on the training dataset but cannot generalize to the test environment.

%\textbf{State Over-specification} Why does the spurious correlations exists in our problem setting? Note that our state space contains multiple modalities, but usually an expert does not need all the modalities to make decisions. For example, to perform the task of \textit{cutting an apple into slices}, the expert decides where to cut based on the shape and size of the apple and probably not based on the texture of the cutting board or the color of the knife handle. Thus, the state is over-specified with some modalities containing extraneous information that was used by the experts to perform the task. We use $\bar{\mathcal{S}}$ to denote all these over-specified modalities and use $\mathcal{S}^*$ to denote modalities really useful for decision making, where $\mathcal{S}^* \times \bar{\mathcal{S}}=\mathcal{S}$ and $\bar{\mathcal{S}}$ and $\mathcal{S}^*$ have no intersection. 


%Such spurious correlation is typically caused by that the $\mathcal{D}_{\text{train}}$ and $\mathcal{D}_{\text{val}}$ only have finite size and cannot cover all the states in $e_\text{test}$ or moreover, there exists a gap between $e_\text{train}$, $e_\text{val}$ and $e_\text{test}$. 

%The expert usually  Let $\mathcal{S}^*$ includes all the modalities that are used by the expert to perform the task, and $\bar{\mathcal{S}}$ as the complimentary modalities where  and $\mathcal{S}^*$  with $\bar{\mathcal{S}}$. The modalities in $\mathcal{S}^*$ are invariant across the 

%$\bar{\mathcal{S}}$ causes the \textbf{state over-specification} problem, 

%In our problem setting, the emergence of spurious correlations is caused by \textbf{state over-specification}, which is the problem that the state observed by the agent contains modalities with extraneous information that was not used by the expert to perform the task. 

\section{Masked Imitation Learning}
\label{sec:method}

%\textbf{Remark 4.} Learning modality masks with additional/validation data is more efficient than directly learning from the validation data in addition to the training data. 

To address overfitting caused by state over-specification, our key insight is to be \textit{selective} about what modalities the policy relies on for deicision making, and remove the over-specified modalities and only preserve the modalities that are generalizable across environments. 
We develop a masked imitation learning (MIL) method to achieve this. %Note that our algorithm is completely \textit{offline}, using only the training dataset $\mathcal{D}_\text{train}$ and the validation dataset $\mathcal{D}_\text{val}$ without any online interactions with the environment.
In this section, we present the model architecture and discuss loss design.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/approach.pdf}
    \caption{\small{Masked imitation learning (MIL) from multimodal data: the inner loop of MIL takes a fixed mask and uses standard behavioral cloning objective to optimize the policy network; and the outer loop of MIL employs a validation loss to update the binary modality mask.}}
    \label{fig:approach}
    \vspace{-0.3cm}
\end{figure*}

\subsection{Policy Network Architecture}
Fig.~\ref{fig:approach} shows an overview of our proposed masked imitation learning (MIL) method. 
Our model consists of three parts: the feature encoder for each modality $G_\theta^i|_{i=1}^{M}$, a learnable binary mask vector $\Psi \in \{0,1\}^M$ with one bit mask for each modality, and an action predictor $F_\theta$. 
We use $\theta$ to denote all the parameters of the encoders $G^i|_{i=1}^{M}$ and the action predictor $F$. 
The feature encoder $G^i$ extract a feature vector $G^i(s^i)$ from the $i$-th modality. Then the feature $G^i(s^i)$ is multiplied by the $i$-th dimension of the mask $\Psi[i]$ and all the masked features are then concatenated into a single feature vector: $[\Psi^1 G^1(s^1), \dots, \Psi^M G^M(s^M)]$, where $F$ uses this masked featurized state to predict the final action. 
In all, our policy can be represented as:
\begin{equation}
    \pi(s;\Psi,\theta) = F_\theta\left([\Psi[1] G_\theta^1(s^1), \dots, \Psi[M] G_\theta^M(s^M)]\right).
\end{equation}



\subsection{Bi-Level Optimization}
The goal of MIL is to simultaneously optimize $G_\theta^i|_{i=1}^{M}$ and $F_\theta$ and find a mask $\Psi$ that assigns zero weight to over-specified modalities. To achieve this, at the high level, we develop a bi-level optimization framework, where the inner-level takes a fixed mask and optimizes $G_\theta^i|_{i=1}^{M}$ and $F_\theta$ with imitation training loss $\mathcal{L}_\text{in}$ using standard gradient descent over $\theta$ and the outer loop optimizes the modality mask $\Psi$ with the validation loss $\mathcal{L}_\text{out}$ using the coordinate descent algorithm~\citep{wright2015coordinate}. 
The key idea of MIL is that the inner-level optimization process could find a model that minimizes the imitation learning loss on the training data for a specific mask, and the outer loop evaluates the generalizability of the learned model with a validation loss and decides whether the mask selects the robust modalities.

Specifically, following the coordinate descent algorithm that is widely used for learning binary variables, we start from a mask $\Psi$ with all the entries as one and iteratively update the mask from the first bit to the last bit cyclicly one bit at a time. 
At each iteration, we have a mask $\Psi$ and a bit index $j$ indicating which bit we want to update in this iteration. We create two masks $\Psi^0$ and $\Psi^1$ by setting the $j$-th bit of $\Psi$ as $0$ and $1$ respectively. We then execute the inner-level imitation learning process for $\Psi^0$ and $\Psi^1$ respectively with the inner-level imitation loss, where we take the widely-adopted L2 loss optimized on the training data $\mathcal{D}_\text{train}$:
\begin{equation}
    \mathcal{L}_\text{in}(\theta) = \mathbb{E}_{(s,a)\in \mathcal{D}_\text{train}}||\pi(s;\Psi,\theta)-a||^2.
\end{equation}
After convergence, we learn the parameters $\theta(\Psi)$ that optimize the imitation learning loss $\mathcal{L}_{\text{in}}$ for the given masks $\Psi^0$ and $\Psi^1$. In the outer loop, after deriving the parameters $\theta(\Psi^0)$ and $\theta(\Psi^1)$ that optimize $\mathcal{L}_{\text{in}}$ for $\Psi^0$ and $\Psi^1$ respectively, we evaluate the generalizability of both parameters with a validation loss with the same form as the training loss but on the validation data $\mathcal{D}_{\text{val}}$:
\begin{equation}\label{eqn:valid}
    \mathcal{L}_\text{out}(\Psi) = \mathbb{E}_{(s,a)\in \mathcal{D}_\text{val}}||\pi(s;\Psi,\theta(\Psi))-a||^2.
\end{equation}
The only difference between $\mathcal{L}_\text{in}$ and $\mathcal{L_\text{out}}$ is the dataset they are trained on, i.e., $\mathcal{D}_\text{train}$ vs. $\mathcal{D}_\text{val}$. The mask that includes  extraneous modalities will overfit to the training data and introduce a high $\mathcal{L}_\text{out}$ on $\mathcal{D}_\text{val}$. Thus, at the $j$-th iteration (corresponding to the $j$-th bit of the mask), we select the mask ($\Psi^0$ or $\Psi^1$) that minimizes the outer loss $\mathcal{L}_\text{out}$ to update the $j$-th bit of mask. We then repeat this procedure to update the next bit in the mask.

\begin{figure}[b]
\vspace{-0.5cm}
 \centering 
    \includegraphics[width=0.36\textwidth]{figures/motivation.pdf}  
  \caption{\small{Motivation for using a state-based loss: Blue policy has a lower action loss compared to Red policy on a given set of states from the validation dataset, but its trajectory starting from the same initial state deviates more from the validation trajectory.}}
  \label{fig:state_loss}
\end{figure}


\noindent \textbf{Remark.} Note that although we adopt similar training and validation loss as common imitation learning algorithms, the modality mask and the bi-level optimization process allow MIL to learn a more generalizable policy. 
In a common imitation learning setting, the policy uses all the modalities and cannot avoid overfitting to extraneous modalities, the validation loss can only select the most generalizable policy within a pool of overfitting policies. However, with MIL, the validation loss selects which mask to use instead of selecting $\theta$, which allows it to remove extraneous modalities that cause overfitting leading to learning a more generalizable imitation policy. 
% Thus, MIL can learn a more generalizable policy than plain imitation learning.



\subsection{Updating Validation Loss Using a Forward Dynamics Model}



\begin{figure*}[btp]
    \centering
    \begin{subfigure}[t]{.2\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=\linewidth]{figures/reacher_two_halves.pdf}
        \caption{\texttt{Reacher}}
        \label{fig:reacher}
        \vspace{0.1cm}
    \end{subfigure}
    \hfil
    \begin{subfigure}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=\linewidth]{figures/task_can.png}
        \caption{\texttt{Robomimic-Can}}
        \label{fig:robomimic-can}
    \end{subfigure}
    \hfil
    \begin{subfigure}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=\linewidth]{figures/square.png}
        \caption{\texttt{Robomimic-Square}}
        \label{fig:robomimic-square}
    \end{subfigure}    
    \hfil
    \begin{subfigure}[t]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=\linewidth]{figures/bookshelf.pdf}
        \caption{\texttt{Bookshelf} (real robot)}
        \label{fig:realrobot}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{Experimental task domains.}
    \label{fig:domains}
    \vspace{-0.4cm}
\end{figure*}


The current validation loss defined on state-action pairs in Eqn.~\eqref{eqn:valid} only evaluates the per-step error of actions. However, as demonstrated in prior works~\cite{ross2011reduction,ross2010efficient}, imitation learning suffers from large compounding errors across long sequences even though the error in each step can be small. As a concrete abstract example, in Fig.~\ref{fig:state_loss}, we have two policies (Red and Blue) each generating a sample trajectory shown in the figure. A sample trajectory from the validation dataset starting from the same initial state is also shown in green. Even though the Blue policy has lower action loss compared to the Red policy, its rollout deviates more from the validation trajectory. Therefore, the per-step validation loss sometimes cannot accurately evaluate the performance of a policy on the validation dataset, which may lead to selecting a suboptimal mask. 
% motivation for state-based loss 
Instead, we would like to use the distance between the policy rollouts and validation trajectories as the validation loss such that Red policy achieves a lower loss than the Blue policy.
% Instead, we need to compute the long-term compounding errors of the whole trajectory.
Since our method is offline, we cannot generate rollouts by interacting with the environment. Instead, we learn a forward dynamics model $\overline{\mathcal{T}}$ to approximate the transition dynamics $\mathcal{T}$ based on $\mathcal{D}_\text{val}$. 
% since $\overline{\mathcal{T}}$ will only be applied to the validation data. 
% The loss to train the forward dynamics model can be derived as follows:
Let us define the forward dynamics loss as:
\begin{equation}
    \mathcal{L}(\overline{\mathcal{T}}) = \mathbb{E}_{(s_t,a_t,s_{t+1})\in \mathcal{D}_\text{val}}\lVert\overline{\mathcal{T}}( s_t,a_t)-s_{t+1}\rVert^2.
\end{equation}
Now, we can create a new trajectory $\bar{\tau}$ by rolling out the policy $\pi(s;\Psi,\theta)$ from an initial state $s_0$ of each trajectory $\tau$ in $\mathcal{D}_{\text{val}}$ with the forward dynamics model $\overline{\mathcal{T}}$ as follows:
\begin{equation}
    \bar{s}_0 = s_0, \quad \bar{s}_{t+1} = \overline{\mathcal{T}}(\bar{s}_t, \pi(\bar{s}_t;\Psi,\theta(\Psi))).
\end{equation}
% where we create a new rollout $\bar{\tau}$ with the same length as $\tau$. 
By rolling out the policy from each initial state in $\mathcal{D}_{\text{val}}$ for the same length as the corresponding trajectory in the validation set, we create a new dataset $\bar{\mathcal{D}}_\text{val}$, within which each state $\bar{s}$ has a corresponding state $s$ in $\mathcal{D}_{\text{val}}$. 
We then compute the outer loop validation loss based on the state differences between $\bar{s}\in \bar{\mathcal{D}}_\text{val}$ and $s\in\mathcal{D}_\text{val}$:
\begin{equation}
    \mathcal{L}_\text{out}(\Psi) = \mathbb{E}_{(\bar{s},s)\in(\bar{\mathcal{D}}_\text{val},\mathcal{D}_\text{val})}\lVert \bar{s}-s\rVert^2.
\end{equation}
This new validation loss using the learned forward dynamics model is designed for tasks with long-horizon trajectories or tasks that consist of multiple stages, which can suffer from large compounding errors. Note that the forward dynamics model suffers less from compounding error because we only query data near the trajectories in the validation set. In practice, we train the forward dynamics model with the proprioception states to avoid having to learn visual dynamics models that can be much less accurate.



\noindent \textbf{Remark.} The key elements of MIL are a bi-level optimization that learns a binary mask in the outer loop using coordinate descent and a learned forward dynamics model for constructing validation loss of long-horizon tasks. 
The full algorithm is presented in Appendix A. 
Note that MIL learns to filter extraneous modalities that induce large generalization errors (high validation loss) but do not necessarily return the smallest number of modalities needed to learn a task. If there are redundant modalities that do not influence the performance of the learned policy (whether it was used by the expert or not), MIL may not learn to filter them. 

